MaxCutPool: differentiable feature-aware Maxcut for pooling in graph neural networks

We propose a novel approach to compute the MAXCUT in attributed graphs, i.e., graphs with features associated with nodes and edges. Our approach works well on any kind of graph topology and can find solutions that jointly optimize the MAXCUT along with other objectives. Based on the obtained MAXCUT partition, we implement a hierarchical graph pooling layer for Graph Neural Networks, which is sparse, trainable end-to-end, and particularly suitable for downstream tasks on heterophilic graphs.

==> algorithms/multipartite_generation.tex <==
\begin{algorithm}[H]
\caption{A multipartite graph generation procedure.}
\label{alg:multipartite}
\begin{algorithmic}
\Require{The number of graph classes $C$}
\Require{The maximum number of nodes per partition $K$}
\Require{The number of graphs per class $N$}
\Ensure{A dataset $D$ of $C$-partite complete graphs}
\State{Let $V$ be the 2D vertices of a regular polygon with $C$ edges.}

\For{$i \gets 1$ to $C$} \Comment{Iterate over classes}
    \State{Apply a rotation permutation on $V$} \Comment{Get the graph class label}
    \State{$T \gets V[0]$}

    \For{$n \gets 1$ to $N$} \Comment{Sample $N$ graphs}

        \State{$S \gets [\,]$} \Comment{The sizes of each partition}
        \For{$j \gets 1$ to $C$}
            State{$S[j] \gets  \text{randint}(K)$}
        \EndFor
        \State{Generate $A$ a $C$-partite complete adjacency matrix.}
        \State{$X \gets [\,]$} \Comment{The node attributes}
        \For{$j \gets 1$ to $C$} \Comment{Sample the coordinates of each node}
            \For{$k \gets 1$ to $S[i]$}
                \State{Sample from $\mathcal{N}(V[j],1)$ the node coordinates $\vx$.}
                \State{Add $\vx$ and $j$ as node attributes.}
            \EndFor
        \EndFor
    \EndFor
    \State{Add $(X,A)$ to the dataset $D$}
\EndFor
% \If{$i \mod S == 0$} \Comment{Sampling each $S$ steps}
% \For{$j \gets 1$ to $V$} \Comment{V validity rejection trials}
% \State{$\boldsymbol{y} \gets $ sample($\boldsymbol{x}_i$)}
% \If{$\boldsymbol{y}$ is valid}
% \State{Add $\boldsymbol{y}$ to $M$ and exit the loop.}
% \EndIf
% \EndFor
\State \Return $D$
\end{algorithmic}
\end{algorithm}

==> complexity_2.tex <==
\subsection{Algorithmic complexity}
\label{app:algo_comp}

The complexity of \gls{diffndp} depends on the complexities of the operations \texttt{SEL}, \texttt{RED}, and \texttt{CON} and the auxiliary loss function.

\subsubsection{\texttt{SEL}}
The complexity of the \texttt{SEL} operation depends on the ScoreNet, which consists of a stack of $L$ \gls{hetmp} layers followed by an \gls{mlp}, and on the auxiliary loss $\mathcal{L}_\text{cut}$.

\paragraph{\gls{hetmp}}
Following the analysis in \cite{blakely2019complexity}, for a graph with $N$ nodes, $E$ edges, and $F$ features, each \gls{hetmp} layer has a time complexity of $\mathcal{O}(NF^2 + EF)$ and a space complexity of $\mathcal{O}(E + NF + F^2)$. This results in a space and time complexity of $\mathcal{O}(N + E)$ with respect to the input.

\paragraph{\gls{mlp}}
The \gls{mlp} has a fixed structure with predetermined layer sizes. Since it operates independently on each node's feature vector and the number of operations per node is constant, processing each node takes $\mathcal{O}(1)$ time. With $N$ nodes to process, this results in a total time complexity of $\mathcal{O}(N)$ with respect to the input. The space complexity is also $\mathcal{O}(N)$, as we need to store the \gls{mlp} hidden and output features for each node.

\subsubsection{\texttt{RED}}
For the non-expressive variant, \texttt{RED} involves a Hadamard product between the scores and features of the $K$ selected nodes, giving a time complexity of $\mathcal{O}(K)$. The expressive variant requires an additional multiplication with the assignment matrix $\mS$, increasing the complexity to $\mathcal{O}(K + ND)$. When $K$ is a function of $N$ (e.g., $K=N/2$), both variants have a time complexity of $\mathcal{O}(N)$ with respect to the input.

The space complexity is $\mathcal{O}(N)$, representing the storage of input and output data.

\subsubsection{\texttt{CON}}
Our efficient implementation of the nearest neighbor assignment follows the complexity of BFS: $\mathcal{O}(N + E)$ time and $\mathcal{O}(N)$ space.

\subsubsection{Loss and total complexity}
The auxiliary loss $\mathcal{L}_\text{cut}$ requires computing a quadratic form, with time complexity $\mathcal{O}(E)$ and space complexity $\mathcal{O}(N+E)$.

\paragraph{Total complexity}
The overall complexity of \gls{diffndp} is:

\begin{equation}
    \label{app:space-time-complex}
    \begin{aligned}
    \text{Time complexity:} &  \;\;\mathcal{O}(E + N) \\
    \text{Space complexity:} & \;\; \mathcal{O}(E + N)
    \end{aligned}
\end{equation}

These sub-quadratic complexities match those of the most efficient \gls{mp} and trainable pooling operators.

==> complexity_old.tex <==
\subsection{Algorithmic complexity}
\label{app:algo_comp}

The complexity of \gls{diffndp} depends on the complexities of the operations \sel{}, \red{}, and \con{} and the loss function.

\subsubsection{\sel}
\paragraph{\gls{hetmp}}
The complexity of the \sel{} operation depends on the ScoreNet, which consists of a stack of $L$ \gls{hetmp} layers followed by an \gls{mlp}, and on the auxiliary loss $\mathcal{L}_\text{cut}$.
We analyze each component in detail in the following.

The time complexity of each \gls{hetmp} is given by applying the trainable parameters $\boldsymbol{\Theta} \in \mathbb{R}^{D \times H}$ to the node features, which costs $\mathcal{O}(NDH)$, and by aggregating the features from neighboring nodes, which costs $\mathcal{O}(EH)$.
Given that we have $L$ layers, the total complexity is $\mathcal{O}\big(L(NDH + EH)\big)$, in general, and $\mathcal{O}(E)$, with respect to the input.

The space complexity of each \gls{hetmp} is given by storing the node features $\mX$, $\mathcal{O}(ND)$, the adjacency matrix $\mA$, $\mathcal{O}(E)$, the parameters $\boldsymbol{\Theta}$ and the activations for the initial, $\mathcal{O}(DH)$, the intermediate, $\mathcal{O}(HH)$, and the last layer, $\mathcal{O}(H)$, respectively, pluse the output $\mX'$, $\mathcal{O}(NH)$.
So, the total space complexity is   
$\mathcal{O}\big(ND + E + H(D + (L-2)H + 1 + N)\big)$, in general, and $\mathcal{O}(E)$, with respect to the input.

\paragraph{\gls{mlp}}
When applying a \gls{mlp} to the output features $\mX'$ of a \gls{hetmp}, the \gls{mlp} operates independently on each node's feature vector. This means the computation is node-wise, and we can calculate the complexities accordingly.
The time complexity is $\mathcal{O}(HH^{(1)})$ for the first layer and $\mathcal{O}(H^{(m-1)}H^{(m)})$ for the remaining layers, where $H^{(m)}$ denotes the size of the $m$-th hidden layer.
If the sum for all layers we get $\mathcal{O}\left(H H^{(1)} + \sum_{m=2}^{M} H^{(m-1)}H^{(m)}\right)$. By multiplying for all the nodes we get that the total complexity is $\mathcal{O}\left(N \times \left(H H^{(1)} + \sum_{m=2}^{M} H^{(m-1)}H^{(m)}\right) \right)$, in general, and $\mathcal{O}(N)$, with respect to the input.

The space complexity is given by the space occupied by the weights and biases $\mW^{(m)}$ and $\vb^{(m)}$ of each layer, which is $\mathcal{O}\left( \sum_{m=1}^{M} H^{(m-1)} H^{(m)} + \sum_{m=1}^{M} H^{(m)} \right)$. In addition, there is the cost of storing the activations at each node.
So, the total cost is $\mathcal{O}\left( \sum_{m=1}^{M} H^{(m-1)} H^{(m)} + N \left( \sum_{m=1}^{M} H^{(m)} \right)\right)$, in general, and $\mathcal{O}(N)$, with respect to the input.

\subsubsection{\red{}}
The \red{} operation for the non-expressive variant is simply a Hadamard product between the scores of the top-$K$ selected nodes and their node features. As such, it has a time complexity of $\mathcal{O}(K)$. 
The expressive variant involves an additional multiplication with the assignment matrix $\mS$, which is however sparse with $N$ non-zero entries.
As such, the time complexity increases to $\mathcal{O}(K + ND)$.
If we let $K$ be a function of $N$, \eg $N/2$, in both cases we have that the time complexity of \red{} with respect to the input is $\mathcal{O}(N)$.

Since there are no intermediate results, the space complexity is only the one necessary to store the input and the output data, which is $\mathcal{O}(N)$.

\subsubsection{\con}
Thanks to the efficient and scalable implementation  discussed in App.~\ref{app:nearest-neighbour}, the space and time complexity of the assignment scheme used to implement the \red{} is the same as the BFS, which is known to have time complexity $\mathcal{O}(N + E)$ and space complexity $\mathcal{O}(N)$.

\subsubsection{Loss and total}

\paragraph{Loss $\mathcal{L}_\text{cut}$}
The cost is that of computing a quadratic form, which has time complexity $\mathcal{O}(E)$ and space complexity $\mathcal{O}(N+E)$.

\paragraph{Total}
So, the overall time complexity of \gls{diffndp} is dominated by the \red{} function, while the space complexity is dominated by the loss function.
%
\begin{equation}
    \label{app:space-time-complex}
    \begin{aligned}
    \text{Time complexity:} &  \qquad \mathcal{O}(E + N) \\
    \text{Space complexity:} & \qquad \mathcal{O}(E + N)
    \end{aligned}
\end{equation}
%
We note that those complexities are sub-quadratic and the number of nodes is the same as the most efficient \gls{mp} and trainable pooling operators.

==> tables/graph_class_hp_merge.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Hyperparameters configurations of the AUX-Net for the graph classification task in both expressive and non-expressive cases.}
\label{tab:graph-class_config_merge}
\begin{tabular}{|l|c|c|c|c|}
\cmidrule[1.5pt]{1-5}
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{Expressive}} & \multicolumn{2}{c|}{\textbf{Non-expressive}} \\
\cline{2-5}
 & MP units & $\beta$ & MP units & $\beta$ \\
\cmidrule[1pt]{1-5}
GCB-H & $[32] \times 8$ & 5.0 & $[8] \times 16$ & 3.0 \\
COLLAB & $[32] \times 8$ & 1.0 & $[32] \times 8$ & 1.0 \\
DD & $[8] \times 16$ & 5.0 & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 \\
ENZYMES & $[16] \times 8$ & 3.0 & $[8] \times 16$ & 3.0 \\
EXPWL1 & $[16] \times 8$ & 1.0 & $[32,32,16,16,8,8]$ & 1.0 \\
MUTAG & $[16] \times 8$ & 3.0 & $[8] \times 16$ & 1.0 \\
Multipartite & $[32] \times 8$ & 1.0 & $[32] \times 8$ & 3.0 \\
Mutagenicity & $[32] \times 8$ & 5.0 & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
NCI1 & $[8] \times 16$ & 3.0 & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
PROTEINS & $[32, 32, 16, 16, 8, 8]$ & 5.0 & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 3.0 \\
REDDIT-B & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 & $[32] \times 8$ & 1.0 \\
\cmidrule[1.5pt]{1-5}
\end{tabular}
\end{table}

==> tables/graph_class_hp_merge_2.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Hyperparameters configurations of the AUX-Net for the graph classification task in both expressive and non-expressive cases.}
\label{tab:graph-class_config_merge}
\begin{tabular}{|l|c|c|c|c|}
\cmidrule[1.5pt]{1-5}
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{MP units}} & \multicolumn{2}{c|}{\textbf{$\beta$}} \\
\cline{2-5}
 & Expressive & Non-expressive & Exp & Non-exp \\
\cmidrule[1pt]{1-5}
GCB-H & $[32] \times 8$ & $[8] \times 16$ & 5.0 & 3.0 \\
COLLAB & $[32] \times 8$ & $[32] \times 8$ & 1.0 & 1.0 \\
DD & $[8] \times 16$ & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 5.0 & 1.0 \\
ENZYMES & $[16] \times 8$ & $[8] \times 16$ & 3.0 & 3.0 \\
EXPWL1 & $[16] \times 8$ & $[32,32,16,16,8,8]$ & 1.0 & 1.0 \\
MUTAG & $[16] \times 8$ & $[8] \times 16$ & 3.0 & 1.0 \\
Multipartite & $[32] \times 8$ & $[32] \times 8$ & 1.0 & 3.0 \\
Mutagenicity & $[32] \times 8$ & $[32, 32, 16, 16, 8, 8]$ & 5.0 & 1.0 \\
NCI1 & $[8] \times 16$ & $[32, 32, 16, 16, 8, 8]$ & 3.0 & 1.0 \\
PROTEINS & $[32, 32, 16, 16, 8, 8]$ & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 5.0 & 3.0 \\
REDDIT-B & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & $[32] \times 8$ & 1.0 & 1.0 \\
\cmidrule[1.5pt]{1-5}
\end{tabular}
\end{table}

==> tables/graph_class_hyperparams.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Hyperparameters configurations of the AUX-Net for the graph classification task in the non expressive case.}
\label{tab:graph-class_config}
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-3}
\textbf{Dataset}     & MP units & $\beta$ \\
\midrule
GCB-H         & $[8] \times 16$ & 3.0 \\
COLLAB       & $[32] \times 8$ & 1.0 \\
DD          & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 \\
ENZYMES & $[8] \times 16$ & 3.0 \\
EXPWL1 & $[32,32,16,16,8,8]$ & 1.0 \\
MUTAG & $[8] \times 16$ & 1.0 \\
Multipartite & $[32] \times 8$ & 3.0 \\
Mutagenicity             & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
NCI1            & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
PROTEINS & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 3.0 \\
REDDIT-B & $[32] \times 8$ & 1.0 \\
\cmidrule[1.5pt]{1-3}
\end{tabular}
\end{table}


==> tables/graph_class_hyperparams_expr.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Hyperparameters configurations of the AUX-Net for the graph classification task in the expressive case.}
\label{tab:graph-class_config_expr}
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-3}
\textbf{Dataset}     & MP units & $\beta$ \\
\midrule
GCB-H         & $[32] \times 8$ & 5.0 \\
COLLAB       & $[32] \times 8$ & 1.0 \\
DD          & $[8] \times 16$ & 5.0 \\
ENZYMES & $[16] \times 8$ & 3.0 \\
EXPWL1 & $[16] \times 8$ & 1.0 \\
MUTAG & $[16] \times 8$ & 3.0 \\
Multipartite & $[32] \times 8$ & 1.0 \\
Mutagenicity & $[32] \times 8$ & 5.0 \\
NCI1 & $[8] \times 16$ & 3.0 \\
PROTEINS & $[32, 32, 16, 16, 8, 8]$ & 5.0 \\
REDDIT-B & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 \\
\cmidrule[1.5pt]{1-3}
\end{tabular}
\end{table}


==> tables/graph_class_res_bw.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.3em} %horizontal padding
\begin{table}[ht]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccccccccccc@{}}
\toprule
Pooling  & GCB-H & COLLAB & DD & ENZYMES & EXPWL1 & MUTAG & Multipart. & Mutagen. & NCI1 & PROTEINS & REDDIT-B \\ 
\midrule
diffpool     & 51{{\tiny$\pm$8}} & 70{{\tiny$\pm$2}} & 77{{\tiny$\pm$4}} & 36{{\tiny$\pm$7}} & 69{{\tiny$\pm$3}}  & 81{{\tiny$\pm$11}} & 9{{\tiny$\pm$1}}   & 78{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 90{{\tiny$\pm$2}} \\
dmon         & 74{{\tiny$\pm$3}} & 68{{\tiny$\pm$2}} & 78{{\tiny$\pm$5}} & 37{{\tiny$\pm$7}} & 73{{\tiny$\pm$3}}  & 82{{\tiny$\pm$11}} & 52{{\tiny$\pm$2}}  & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$2}} & 76{{\tiny$\pm$4}} & 88{{\tiny$\pm$2}} \\
edgepool     & 75{{\tiny$\pm$4}} & 72{{\tiny$\pm$3}} & 73{{\tiny$\pm$5}} & 35{{\tiny$\pm$8}} & 90{{\tiny$\pm$2}}  & 84{{\tiny$\pm$12}} & 55{{\tiny$\pm$3}}  & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$3}} & 74{{\tiny$\pm$5}} & 91{{\tiny$\pm$2}} \\
graclus      & 75{{\tiny$\pm$3}} & 72{{\tiny$\pm$3}} & 73{{\tiny$\pm$4}} & 33{{\tiny$\pm$7}} & 90{{\tiny$\pm$2}}  & 82{{\tiny$\pm$12}} & 25{{\tiny$\pm$18}} & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$2}} & 73{{\tiny$\pm$4}} & 90{{\tiny$\pm$3}} \\
kmis         & 75{{\tiny$\pm$4}} & 71{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 33{{\tiny$\pm$8}} & 99{{\tiny$\pm$1}}  & 83{{\tiny$\pm$10}} & 58{{\tiny$\pm$2}}  & 79{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 73{{\tiny$\pm$5}} & 90{{\tiny$\pm$2}} \\
mincut       & 75{{\tiny$\pm$5}} & 70{{\tiny$\pm$2}} & 78{{\tiny$\pm$5}} & 34{{\tiny$\pm$9}} & 71{{\tiny$\pm$3}}  & 81{{\tiny$\pm$12}} & 56{{\tiny$\pm$3}}  & 78{{\tiny$\pm$3}} & 73{{\tiny$\pm$3}} & 77{{\tiny$\pm$5}} & 87{{\tiny$\pm$2}} \\
topk         & 56{{\tiny$\pm$5}} & 72{{\tiny$\pm$2}} & 72{{\tiny$\pm$5}} & 29{{\tiny$\pm$7}} & 73{{\tiny$\pm$2}}  & 82{{\tiny$\pm$10}} & 43{{\tiny$\pm$3}}  & 75{{\tiny$\pm$3}} & 73{{\tiny$\pm$2}} & 74{{\tiny$\pm$5}} & 77{{\tiny$\pm$2}} \\
\midrule
diffndp      & 73{{\tiny$\pm$3}} & 77{{\tiny$\pm$2}} & 77{{\tiny$\pm$4}} & 31{{\tiny$\pm$6}} & 100{{\tiny$\pm$1}} & 84{{\tiny$\pm$10}} & 90{{\tiny$\pm$2}}  & 77{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & 74{{\tiny$\pm$4}} & 89{{\tiny$\pm$3}} \\
diffndp-e & 74{{\tiny$\pm$3}} & 77{{\tiny$\pm$2}} & 77{{\tiny$\pm$3}} & 34{{\tiny$\pm$5}} & 100{{\tiny$\pm$0}} & 85{{\tiny$\pm$9}}  & 87{{\tiny$\pm$5}}  & 79{{\tiny$\pm$1}} & 76{{\tiny$\pm$2}} & 74{{\tiny$\pm$4}} & 89{{\tiny$\pm$2}} \\ 
\midrule
diffndp-nl & 61{{\tiny$\pm$6}} & 77{{\tiny$\pm$3}} & 74{{\tiny$\pm$4}} & 31{{\tiny$\pm$4}} & 100{{\tiny$\pm$0}} & 83{{\tiny$\pm$11}} & 91{{\tiny$\pm$1}} & 76{{\tiny$\pm$3}} & 74{{\tiny$\pm$2}} & 70{{\tiny$\pm$4}} & 86{{\tiny$\pm$3}} \\

\bottomrule
\end{tabular}
}
\caption{Graph classification accuracy values}
\label{tab:graph-classification}
\end{table}
\egroup

==> tables/graph_class_res_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.3em} %horizontal padding
\begin{table}[ht]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccccccccccc@{}}
\toprule
Pooling  & GCB-H & COLLAB & DD & ENZYMES & EXPWL1 & MUTAG & Multipart. & Mutagen. & NCI1 & PROTEINS & REDDIT-B \\
\midrule
 no pool     & 74{{\tiny$\pm$4}} & 74{{\tiny$\pm$2}} & 73{{\tiny$\pm$5}} & 33{{\tiny$\pm$6}} & 87{{\tiny$\pm$2}}  & 78{{\tiny$\pm$13}} & 14{{\tiny$\pm$12}} & 79{{\tiny$\pm$2}} & 78{{\tiny$\pm$3}} & 71{{\tiny$\pm$4}} & 90{{\tiny$\pm$2}}\\ 
\midrule
diffpool     & 51{{\tiny$\pm$8}} & 70{{\tiny$\pm$2}} & 77{{\tiny$\pm$4}} & 36{{\tiny$\pm$7}} & 69{{\tiny$\pm$3}}  & 81{{\tiny$\pm$11}} & 9{{\tiny$\pm$1}}   & 78{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 90{{\tiny$\pm$2}} \\
dmon         & 74{{\tiny$\pm$3}} & 68{{\tiny$\pm$2}} & 78{{\tiny$\pm$5}} & 37{{\tiny$\pm$7}} & 73{{\tiny$\pm$3}}  & 82{{\tiny$\pm$11}} & 52{{\tiny$\pm$2}}  & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$2}} & 76{{\tiny$\pm$4}} & 88{{\tiny$\pm$2}} \\
edgepool     & 75{{\tiny$\pm$4}} & 72{{\tiny$\pm$3}} & 73{{\tiny$\pm$5}} & 35{{\tiny$\pm$8}} & 90{{\tiny$\pm$2}}  & 84{{\tiny$\pm$12}} & 55{{\tiny$\pm$3}}  & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$3}} & 74{{\tiny$\pm$5}} & 91{{\tiny$\pm$2}} \\
graclus      & 75{{\tiny$\pm$3}} & 72{{\tiny$\pm$3}} & 73{{\tiny$\pm$4}} & 33{{\tiny$\pm$7}} & 90{{\tiny$\pm$2}}  & 82{{\tiny$\pm$12}} & 25{{\tiny$\pm$18}} & 80{{\tiny$\pm$2}} & 77{{\tiny$\pm$2}} & 73{{\tiny$\pm$4}} & 90{{\tiny$\pm$3}} \\
kmis         & 75{{\tiny$\pm$4}} & 71{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 33{{\tiny$\pm$8}} & 99{{\tiny$\pm$1}}  & 83{{\tiny$\pm$10}} & 58{{\tiny$\pm$2}}  & 79{{\tiny$\pm$2}} & 75{{\tiny$\pm$3}} & 73{{\tiny$\pm$5}} & 90{{\tiny$\pm$2}} \\
mincut       & 75{{\tiny$\pm$5}} & 70{{\tiny$\pm$2}} & 78{{\tiny$\pm$5}} & 34{{\tiny$\pm$9}} & 71{{\tiny$\pm$3}}  & 81{{\tiny$\pm$12}} & 56{{\tiny$\pm$3}}  & 78{{\tiny$\pm$3}} & 73{{\tiny$\pm$3}} & 77{{\tiny$\pm$5}} & 87{{\tiny$\pm$2}} \\
topk         & 56{{\tiny$\pm$5}} & 72{{\tiny$\pm$2}} & 72{{\tiny$\pm$5}} & 29{{\tiny$\pm$7}} & 73{{\tiny$\pm$2}}  & 82{{\tiny$\pm$10}} & 43{{\tiny$\pm$3}}  & 75{{\tiny$\pm$3}} & 73{{\tiny$\pm$2}} & 74{{\tiny$\pm$5}} & 77{{\tiny$\pm$2}} \\
\midrule
diffndp      & 73{{\tiny$\pm$3}} & 77{{\tiny$\pm$2}} & 77{{\tiny$\pm$4}} & 31{{\tiny$\pm$6}} & 100{{\tiny$\pm$1}} & 84{{\tiny$\pm$10}} & 90{{\tiny$\pm$2}}  & 77{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & 74{{\tiny$\pm$4}} & 89{{\tiny$\pm$3}} \\
diffndp-e & 74{{\tiny$\pm$3}} & 77{{\tiny$\pm$2}} & 77{{\tiny$\pm$3}} & 34{{\tiny$\pm$5}} & 100{{\tiny$\pm$0}} & 85{{\tiny$\pm$9}}  & 87{{\tiny$\pm$5}}  & 79{{\tiny$\pm$1}} & 76{{\tiny$\pm$2}} & 74{{\tiny$\pm$4}} & 89{{\tiny$\pm$2}} \\ 
\midrule
diffndp-nl & 61{{\tiny$\pm$6}} & 77{{\tiny$\pm$3}} & 74{{\tiny$\pm$4}} & 31{{\tiny$\pm$4}} & 100{{\tiny$\pm$0}} & 83{{\tiny$\pm$11}} & 91{{\tiny$\pm$1}} & 76{{\tiny$\pm$3}} & 74{{\tiny$\pm$2}} & 70{{\tiny$\pm$4}} & 86{{\tiny$\pm$3}} \\

\bottomrule
\end{tabular}
}
\caption{Graph classification accuracy values}
\label{tab:graph-classification-full}
\end{table}
\egroup

==> tables/graph_class_res_remaining.tex <==
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.8em} %horizontal padding
\begin{table}[ht]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|cccc@{}}
\cmidrule[1.5pt]{1-5}
\textbf{Pooler}  & \textbf{DD} & \textbf{MUTAG} & \textbf{ENZYMES} & \textbf{PROTEINS} \\
\midrule
No pool     & 73{{\tiny$\pm$5}} & 78{{\tiny$\pm$13}} & 33{{\tiny$\pm$6}} & 71{{\tiny$\pm$4}} \\
\midrule
Diffpool    & 77{{\tiny$\pm$4}} & 81{{\tiny$\pm$11}} & 36{{\tiny$\pm$7}} & 75{{\tiny$\pm$3}} \\
\gls{dmon}        & 78{{\tiny$\pm$5}} & 82{{\tiny$\pm$11}} & 37{{\tiny$\pm$7}} & 76{{\tiny$\pm$4}} \\
\gls{ecpool}    & 73{{\tiny$\pm$5}} & 84{{\tiny$\pm$12}} & 35{{\tiny$\pm$8}} & 74{{\tiny$\pm$5}} \\
Graclus     & 73{{\tiny$\pm$4}} & 82{{\tiny$\pm$12}} & 33{{\tiny$\pm$7}} & 73{{\tiny$\pm$4}} \\
\gls{kmis}        & 75{{\tiny$\pm$3}} & 83{{\tiny$\pm$10}} & 33{{\tiny$\pm$8}} & 73{{\tiny$\pm$5}} \\
\gls{mincut}      & 78{{\tiny$\pm$5}} & 81{{\tiny$\pm$12}} & 34{{\tiny$\pm$9}} & 77{{\tiny$\pm$5}} \\
\gls{topk}         & 72{{\tiny$\pm$5}} & 82{{\tiny$\pm$10}} & 29{{\tiny$\pm$7}} & 74{{\tiny$\pm$5}} \\
\midrule
\gls{diffndp}      & 77{{\tiny$\pm$4}} & 84{{\tiny$\pm$10}} & 31{{\tiny$\pm$6}} & 74{{\tiny$\pm$4}} \\
\gls{diffndp}-E   & 77{{\tiny$\pm$3}} & 85{{\tiny$\pm$9}}  & 34{{\tiny$\pm$5}} & 74{{\tiny$\pm$4}} \\
\midrule
\gls{diffndp}-NL  & 74{{\tiny$\pm$4}} & 83{{\tiny$\pm$11}} & 31{{\tiny$\pm$4}} & 70{{\tiny$\pm$4}} \\
\cmidrule[1.5pt]{1-5}
\end{tabular}
}
\caption{\small Graph classification accuracy values (subset)}
\label{tab:graph-classification-subset}
\end{table}
\egroup

==> tables/graph_class_stats.tex <==
% :::::::::::::::::::::::::::: DATASET CLASS ::::::::::::::::::::::::::::
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.5em} %horizontal padding
\begin{table}[!ht]
\small
\centering
\begin{tabular}{l|ccccccc}
\cmidrule[1.5pt]{1-8}
\textbf{Dataset} & \textbf{\#Samples} & \textbf{\#Classes} & \textbf{Avg. \#vertices} & \textbf{Avg. \#edges} & \textbf{V. attr.} & \textbf{V. labels} & $\boldsymbol{\bar h(\gG)}$ \\
\cmidrule[.5pt]{1-8}
EXPWL1        & 3,000  & 2  & 76.96  & 186.46    & --  & yes & 0.2740 \\
NCI1          & 4,110  & 2  & 29.87  & 64.60     & --  & yes & 0.6245 \\
PROTEINS      & 1,113  & 2  & 39.06  & 72.82     & 1   & yes & 0.6582 \\
Mutagenicity  & 4,337  & 2  & 30.32  & 61.54     & --  & yes & 0.3679 \\
COLLAB        & 5,000  & 3  & 74.49  & 4,914.43  & --  & no  & 1 \\ 
REDDIT-B      & 2,000  & 2  & 429.63 & 995.51    & --  & no  & 1 \\
GCB-H         & 1,800  & 3  & 148.32 & 572.32    & --  & yes & 0.8440 \\
DD            & 1,178  & 2  & 284.32 & 1,431.32  & --  & yes & 0.0688 \\
MUTAG         & 188    & 2  & 17.93  & 19.79     & --  & yes & 0.7082 \\
ENZYMES       & 600    & 6  & 32.63  & 62.14     & 18  & yes & 0.6687 \\
Multipartite  & 5000   & 10 &  99.79 & 4,477.43   & 3   & yes & 0.1101\\
\cmidrule[1.5pt]{1-8}
\end{tabular}
\caption{\small Details of the graph classification datasets.} 
\label{tab:gc_dataset}
\end{table}

\egroup
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::



==> tables/graph_class_student_fixed.tex <==
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.3em} %horizontal padding
\begin{table}[ht]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccccccc|c@{}}
\cmidrule[1.5pt]{1-9}
\textbf{Pooler}  & \textbf{GCB-H} & \textbf{COLLAB} & \textbf{EXPWL1} & \textbf{Multipart.} & \textbf{Mutagen.} & \textbf{NCI1} & \textbf{REDDIT-B} & \textbf{Score} \\
\midrule[1pt]
No pool     & \textcolor{gray}{\textit{74{{\tiny$\pm$4}}}} & \textcolor{gray}{\textit{74{{\tiny$\pm$2}}}} & \textcolor{gray}{\textit{ 87{{\tiny$\pm$2}}}}  & \textcolor{gray}{\textit{ 14{{\tiny$\pm$12}}}} & \textcolor{gray}{\textit{79{{\tiny$\pm$2}}}} & \textcolor{gray}{\textit{78{{\tiny$\pm$3}}}} & \textcolor{gray}{\textit{90{{\tiny$\pm$2}}}} & -\\ 
\midrule
DiffPool     & \textcolor{black}{51{{\tiny$\pm$8}}} & \textcolor{black}{70{{\tiny$\pm$2}}} & \textcolor{black}{69{{\tiny$\pm$3}}}  & \textcolor{black}{9{{\tiny$\pm$1}}}   & 78{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}} & 1 \\
\gls{dmon}         & \textcolor{darkgreen}{74{{\tiny$\pm$3}}} & \textcolor{black}{68{{\tiny$\pm$2}}} & \textcolor{black}{73{{\tiny$\pm$3}}}  & \textcolor{black}{52{{\tiny$\pm$2}}}  & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & 88{{\tiny$\pm$2}}& 3 \\
EdgePool     & \textcolor{darkgreen}{75{{\tiny$\pm$4}}} & \textcolor{black}{72{{\tiny$\pm$3}}} & 90{{\tiny$\pm$2}}  & 55{{\tiny$\pm$3}}  & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & \textcolor{darkgreen}{77{{\tiny$\pm$3}}} & \textcolor{darkgreen}{91{{\tiny$\pm$2}}} & 4 \\
Graclus      & \textcolor{darkgreen}{75{{\tiny$\pm$3}}} & \textcolor{black}{72{{\tiny$\pm$3}}} & 90{{\tiny$\pm$2}}  & \textcolor{black}{25{{\tiny$\pm$18}}} & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & \textcolor{darkgreen}{90{{\tiny$\pm$3}}} & 4 \\
\gls{kmis}        & \textcolor{darkgreen}{75{{\tiny$\pm$4}}} & \textcolor{black}{71{{\tiny$\pm$2}}} & \textcolor{darkgreen}{99{{\tiny$\pm$1}}}  & 58{{\tiny$\pm$2}} & \textcolor{darkgreen}{79{{\tiny$\pm$2}}} & 75{{\tiny$\pm$3}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}} & 4 \\
\gls{mincut}       & \textcolor{darkgreen}{75{{\tiny$\pm$5}}} & \textcolor{black}{70{{\tiny$\pm$2}}} & \textcolor{black}{71{{\tiny$\pm$3}}}  & 56{{\tiny$\pm$3}}  & 78{{\tiny$\pm$3}} & \textcolor{black}{73{{\tiny$\pm$3}}} & \textcolor{black}{87{{\tiny$\pm$2}}} & 1 \\
\gls{topk}         & \textcolor{black}{56{{\tiny$\pm$5}}} & \textcolor{black}{72{{\tiny$\pm$2}}} & \textcolor{black}{73{{\tiny$\pm$2}}}  & \textcolor{black}{43{{\tiny$\pm$3}}}  & \textcolor{black}{75{{\tiny$\pm$3}}} & \textcolor{black}{73{{\tiny$\pm$2}}} & \textcolor{black}{77{{\tiny$\pm$2}}} & 0\\
\midrule
\gls{diffndp}      & \textcolor{darkgreen}{73{{\tiny$\pm$3}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & \textcolor{darkgreen}{100{{\tiny$\pm$0}}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}}  & 77{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & \textcolor{darkgreen}{89{{\tiny$\pm$3}}} & 5 \\
\gls{diffndp}-E & \textcolor{darkgreen}{74{{\tiny$\pm$3}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & \textcolor{darkgreen}{100{{\tiny$\pm$0}}} & \textcolor{darkgreen}{87{{\tiny$\pm$5}}}  & \textcolor{darkgreen}{79{{\tiny$\pm$1}}} & \textcolor{darkgreen}{76{{\tiny$\pm$2}}} & \textcolor{darkgreen}{89{{\tiny$\pm$2}}} & \textbf{7}\\ 
\midrule
\gls{diffndp}-NL & \textcolor{black}{61{{\tiny$\pm$6}}} & \textcolor{darkgreen}{77{{\tiny$\pm$3}}} & \textcolor{darkgreen}{100{{\tiny$\pm$0}}} & \textcolor{darkgreen}{91{{\tiny$\pm$1}}} & \textcolor{black}{76{{\tiny$\pm$3}}} & \textcolor{black}{74{{\tiny$\pm$2}}} & \textcolor{black}{86{{\tiny$\pm$3}}} & 3 \\
\cmidrule[1.5pt]{1-9}
\end{tabular}
}
\caption{\small Mean and standard deviations of the graph classification accuracy values. For each dataset the best performing method and those that are not significantly different from it are colored in green.
If a method is in the top-performing group is assigned a score of 1, 0 otherwise.}
\label{tab:graph-classification}
\end{table}
\egroup

==> tables/graph_class_tukey.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.3em} %horizontal padding
\begin{table}[ht]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccccccc|c@{}}
\toprule[1pt]
Pooler  & GCB-H & COLLAB & EXPWL1 & Multipart. & Mutagen. & NCI1 & REDDIT-B & Score\\
\midrule[1pt]
No pool     & \textit{74{{\tiny$\pm$4}} }& \textit{74{{\tiny$\pm$2}}} &\textit{ 87{{\tiny$\pm$2}}}  &\textit{ 14{{\tiny$\pm$12}}} & \textit{79{{\tiny$\pm$2}}} &\textit{ 78{{\tiny$\pm$3}}} & \textit{90{{\tiny$\pm$2}}} & -\\ 
\midrule[1pt]
DiffPool     & \textcolor{darkred}{51{{\tiny$\pm$8}}} & \textcolor{darkred}{70{{\tiny$\pm$2}}} & \textcolor{darkred}{69{{\tiny$\pm$3}}}  & \textcolor{darkred}{9{{\tiny$\pm$1}}}   & 78{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}} & 4\\
\gls{dmon}         & \textcolor{darkgreen}{74{{\tiny$\pm$3}}} & \textcolor{darkred}{68{{\tiny$\pm$2}}} & \textcolor{darkred}{73{{\tiny$\pm$3}}}  & \textcolor{darkred}{52{{\tiny$\pm$2}}}  & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & 77{{\tiny$\pm$2}} & 88{{\tiny$\pm$2}}& 6 \\
EdgePool     & \textcolor{darkgreen}{75{{\tiny$\pm$4}}} & \textcolor{darkred}{72{{\tiny$\pm$3}}} & 90{{\tiny$\pm$2}}  & 55{{\tiny$\pm$3}}  & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & \textcolor{darkgreen}{77{{\tiny$\pm$3}}} & \textcolor{darkgreen}{91{{\tiny$\pm$2}}} & 10 \\
Graclus      & \textcolor{darkgreen}{75{{\tiny$\pm$3}}} & \textcolor{darkred}{72{{\tiny$\pm$3}}} & 90{{\tiny$\pm$2}}  & \textcolor{darkred}{25{{\tiny$\pm$18}}} & \textcolor{darkgreen}{80{{\tiny$\pm$2}}} & 77{{\tiny$\pm$2}} & \textcolor{darkgreen}{90{{\tiny$\pm$3}}} & 8 \\
\gls{kmis}        & \textcolor{darkgreen}{75{{\tiny$\pm$4}}} & \textcolor{darkred}{71{{\tiny$\pm$2}}} & \textcolor{darkgreen}{99{{\tiny$\pm$1}}}  & 58{{\tiny$\pm$2}} & \textcolor{darkgreen}{79{{\tiny$\pm$2}}} & 75{{\tiny$\pm$3}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}} & 10 \\
\gls{mincut}       & \textcolor{darkgreen}{75{{\tiny$\pm$5}}} & \textcolor{darkred}{70{{\tiny$\pm$2}}} & \textcolor{darkred}{71{{\tiny$\pm$3}}}  & 56{{\tiny$\pm$3}}  & 78{{\tiny$\pm$3}} & 73{{\tiny$\pm$3}} & \textcolor{darkgreen}{87{{\tiny$\pm$2}}} & 7 \\
\gls{topk}         & \textcolor{darkred}{56{{\tiny$\pm$5}}} & \textcolor{darkred}{72{{\tiny$\pm$2}}} & \textcolor{darkred}{73{{\tiny$\pm$2}}}  & \textcolor{darkred}{43{{\tiny$\pm$3}}}  & \textcolor{darkred}{75{{\tiny$\pm$3}}} & \textcolor{darkred}{73{{\tiny$\pm$2}}} & \textcolor{darkred}{77{{\tiny$\pm$2}}} & 0\\
\midrule
\gls{diffndp}      & \textcolor{darkgreen}{73{{\tiny$\pm$3}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & \textcolor{darkgreen}{100{{\tiny$\pm$1}}} & \textcolor{darkgreen}{90{{\tiny$\pm$2}}}  & 77{{\tiny$\pm$2}} & 75{{\tiny$\pm$2}} & \textcolor{darkgreen}{89{{\tiny$\pm$3}}} & \textbf{12} \\
\gls{diffndp}-E & \textcolor{darkgreen}{74{{\tiny$\pm$3}}} & \textcolor{darkgreen}{77{{\tiny$\pm$2}}} & \textcolor{darkgreen}{100{{\tiny$\pm$0}}} & \textcolor{darkgreen}{87{{\tiny$\pm$5}}}  & 79{{\tiny$\pm$1}} & 76{{\tiny$\pm$2}} & \textcolor{darkgreen}{89{{\tiny$\pm$2}}} & \textbf{12}\\ 
\midrule
\gls{diffndp}-NL & \textcolor{darkred}{61{{\tiny$\pm$6}}} & \textcolor{darkgreen}{77{{\tiny$\pm$3}}} & \textcolor{darkgreen}{100{{\tiny$\pm$0}}} & \textcolor{darkgreen}{91{{\tiny$\pm$1}}} & 76{{\tiny$\pm$3}} & \textcolor{darkred}{74{{\tiny$\pm$2}}} & 86{{\tiny$\pm$3}} & 8 \\

\bottomrule[1pt]
\end{tabular}
}
\caption{Graph classification accuracy values. The three performance groups (best, mid and worst) are coloured in green, black and red respectively. The groups are assigned a score of 2, 1, 0 points to better visualize the ranking of each pooling method.}
\label{tab:graph-classification}
\end{table}
\egroup

==> tables/maxcut_dataset.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Statistics of the PyGSP datasets used to compute the \maxcut.}
\label{tab:maxcut_dataset}
\subfloat[PyGSP datasets]{
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-4}
\textbf{Dataset}     & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{\# Vertex attr.} \\
\midrule
Barabasi-Albert & 100 & 768 & 2 \\
Community & 90 & 532 & 2 \\
Erdős-Renyi & 100 & 974 & 2 \\
Grid2d (10$\times$10) & 100 & 360 & 2 \\
Grid2d (60$\times$40) & 2,400 & 9400 & 2 \\
Minnesota & 2642 & 6608 & 2 \\
RandRegular & 500 & 1500 & 2 \\
Ring & 100 & 200 & 2 \\
Sensor & 64 & 640 & 2 \\
\cmidrule[1.5pt]{1-4}
\end{tabular}
}
\quad
\subfloat[Gset]{
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-4}
\textbf{Dataset}     & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{\# Vertex attr.} \\
\midrule
G14 & $800$ & $4,694$ & -- \\
G15 & $800$ & $4,661$ & -- \\
G22 & $2,000$ & $19,990$ & -- \\
G49 & $3,000$ & $6,000$ & -- \\
G50 & $3,000$ & $6,000$ & -- \\
G55 & $5,000$ & $12,468$ & -- \\
G70 & $10,000$ & $9,999$ & -- \\
\cmidrule[1.5pt]{1-4}
\end{tabular}
}
\end{table}

==> tables/maxcut_hyperparams.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Hyperparameters configurations of the AUX-Net for the \maxcut task.}
\label{tab:cut_config}
\begin{tabular}{lccccc}
\cmidrule[1.5pt]{1-4}
\textbf{Dataset}     & MP units & MP Act & $\delta$ \\
\midrule
G14        & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & ReLU & 2.0 \\
G15        & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & ReLU & 2.0 \\
G22        & $[4] \times 32$ & Tanh & 2.0 \\
G49        & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & Tanh & 2.0 \\
G50        & $[8] \times 16$ & ReLU & 2.0 \\
G55        & $[4] \times 32$ & ReLU & 2.0 \\
G70        & $[8] \times 16$ & ReLU & 2.0 \\
BarabasiAlbert        & $[4] \times 32$ & Tanh & 2.0 \\
Community        & $[4] \times 32$ & Tanh & 2.0 \\
ErdősRenyi        & $[4] \times 32$ & Tanh & 2.0 \\
Grid2d (10$\times$10)        & $[4] \times 32$ & Tanh & 2.0 \\
Grid2d (60$\times$40)        & $[4] \times 32$ & ReLU & 2.0 \\
Minnesota        & $[4] \times 32$ & Tanh & 2.0 \\
RandRegular        & $[4] \times 32$ & Tanh & 2.0 \\
Ring        & $[4] \times 32$ & ReLU & 2.0 \\
Sensor        & $[4] \times 32$ & Tanh & 2.0 \\
\cmidrule[1.5pt]{1-4}
\end{tabular}
\end{table}


==> tables/maxcut_res.tex <==
\begin{table}[ht]
\fontfamily{bch}\selectfont
\centering
\footnotesize

\subfloat[PyGSP datasets]{

\begin{tabular}{@{}l|cccc@{}}
\cmidrule[1.5pt]{1-5}
Dataset        & GW              & NDP             & GCN    & \gls{diffndp} \\ \midrule
BarabasiAlbert & 0.6875          & 0.6589          & 0.7240 & \textbf{0.7292}                \\
Community      & 0.6767          & 0.6429          & 0.6805 & \textbf{0.6814}                \\
ErdősRenyi     & 0.6920          & 0.6858          & 0.6797 & \textbf{0.7105}                \\
Grid2d (10$\times$10) & \textbf{1.0000} & \textbf{1.0000} & 0.9222 & \textbf{1.0000}                \\
Grid2d (60$\times$40) & -               & 0.9787          & 0.1862 & \textbf{0.9815}                \\
Minnesota      & -               & 0.9104          & 0.8904 & \textbf{0.9130}                \\
RandRegular  & 0.4827               & 0.8760          & 0.8733 & \textbf{0.9040}                \\
Ring           & \textbf{1.0000}               & \textbf{1.0000} & 0.4200 & \textbf{1.0000}                \\
Sensor         & 0.6000          & 0.5719          & 0.6281 & \textbf{0.6406}                \\ 
\cmidrule[1.5pt]{1-5}
\end{tabular}
  }
\quad
\subfloat[GSet datasets]{
\begin{tabular}{@{}l|ccc@{}}
\cmidrule[1.5pt]{1-4}
Dataset & NDP             & GCN    & \gls{diffndp} \\ \midrule
G14     & 0.6155          & 0.6323 & \textbf{0.6412}                \\
G15     & 0.5945          & 0.6288 & \textbf{0.6424}                \\
G22     & 0.6441          & 0.6409 & \textbf{0.6577}                \\
G49     & \textbf{1.0000} & 0.9683 & \textbf{1.0000}                \\
G50     & \textbf{0.9800} & 0.9610 & 0.9750                         \\
G55     & 0.7568          & 0.7865 & \textbf{0.8068}                \\
G70     & 0.8803          & 0.8945 & \textbf{0.9086}                \\ \cmidrule[1.5pt]{1-4}
\end{tabular}
}
%}
\caption{\small Size of the graph cuts obtained with \gls{diffndp}, a \gls{gnn} with \gls{gcn} layers, and two common algorithms to compute the \maxcut. GW results are absent for some entries of the PyGSP datasets and for GSet because the solver failed to converge.}
\label{tab:maxcut}
\end{table}

==> tables/maxcut_res_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.3em} %horizontal padding
\begin{table}[]
\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccc@{}}
\toprule
Dataset        & GW     & NDP    & DiffNDP \\ \midrule
BarabasiAlbert & 0.6875 & 0.6589 & 0.7292  \\
Community      & 0.6767 & 0.6429 & 0.6814  \\
ErdosRenyi     & 0.6920 & 0.6858 & 0.7105  \\
Grid2d         & 1.0000 & 1.0000 & 1.0000  \\
Minnesota      & -      & 0.9104 & 0.9130  \\
RandomRegular  & -      & 0.8760 & 0.9040  \\
Ring           & -      & 1.0000 & 1.0000  \\
Sensor         & 0.6000 & 0.5719 & 0.6406  \\
G14            & -      & 0.6155 & 0.6412  \\
G15            & -      & 0.5945 & 0.6424  \\
G22            & -      & 0.6441 & 0.6577  \\
G49            & -      & 1.0000 & 1.0000  \\
G50            & -      & 0.9800 & 0.9750  \\
G55            & -      & 0.7568 & 0.8068  \\
G70            & -      & 0.8803 & 0.9086  \\ \bottomrule
\end{tabular}
}
\caption{Evaluation of maxcut loss}
\label{tab:maxcut}
\end{table}
\egroup

==> tables/node_class_cat_res.tex <==
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.5em} %horizontal padding
\begin{table}[ht]

\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|cccccc@{}}
\cmidrule[1.5pt]{1-7}
\textbf{Pooler} & \textbf{Roman-empire} & \textbf{Amazon-ratings} & \textbf{Minesweeper}$^{*}$ & \textbf{Tolokers} & \textbf{Questions} & \textbf{Score} \\ 
\midrule
\gls{topk}    & 20{\tiny$\pm$11} & 49{\tiny$\pm$7} & 91{{\tiny$\pm$1}} & \textcolor{darkgreen}{96{{\tiny$\pm$0}}} & 70{{\tiny$\pm$3}} & 1 \\
\gls{kmis}    & 19{\tiny$\pm$2}  & \textcolor{darkgreen}{53{\tiny$\pm$3}} & 90{{\tiny$\pm$0}} & 91{{\tiny$\pm$2}} & \textcolor{darkgreen}{82{{\tiny$\pm$4}}} & 2 \\
\gls{ndp}     & 19{\tiny$\pm$4}  & \textcolor{darkgreen}{56{\tiny$\pm$5}} & \textcolor{darkgreen}{94{{\tiny$\pm$0}}} & 90{{\tiny$\pm$8}} & 69{{\tiny$\pm$7}} & 2 \\
\gls{diffndp} & \textcolor{darkgreen}{67{\tiny$\pm$2}}  & 53{\tiny$\pm$1} & 92{{\tiny$\pm$1}} & \textcolor{darkgreen}{96{{\tiny$\pm$1}}} & \textcolor{darkgreen}{82{{\tiny$\pm$2}}} & \textbf{3} \\
\cmidrule[1.5pt]{1-7}
\end{tabular}
}
\caption{\small Node classification accuracy (Roman-empire, Amazon-ratings) and AUROC (Minesweeper, Tolokers, Questions) obtained when using the architecture with skip connections.}
\label{tab:node-classification-cat}
\end{table}
\egroup

==> tables/node_class_res.tex <==
\bgroup
\def\arraystretch{.8} %vertical padding
\setlength\tabcolsep{.5em} %horizontal padding
\begin{table}[ht]

\makebox[\textwidth]{
\fontfamily{bch}\selectfont
\centering
\footnotesize
\begin{tabular}{@{}l|ccccc|c@{}}
\cmidrule[1.5pt]{1-7}
\textbf{Pooler} & \textbf{Roman-empire} & \textbf{Amazon-ratings} & \textbf{Minesweeper} & \textbf{Tolokers} & \textbf{Questions} & \textbf{Score} \\ 
\midrule
\gls{topk}      & 26{\tiny$\pm$7} & 46{\tiny$\pm$4} & 94{\tiny$\pm$1} & \textcolor{darkgreen}{89{\tiny$\pm$5}} & 64{\tiny$\pm$3} & 1 \\
\gls{kmis}      & 23{\tiny$\pm$3} & 48{\tiny$\pm$2} & 75{\tiny$\pm$2} & 84{\tiny$\pm$2} & \textcolor{darkgreen}{83{\tiny$\pm$1}} & 1 \\
\gls{ndp}       & 22{\tiny$\pm$5} & \textcolor{darkgreen}{53{\tiny$\pm$2}} & \textcolor{darkgreen}{98{\tiny$\pm$0}} & \textcolor{darkgreen}{88{\tiny$\pm$6}} & 68{\tiny$\pm$4} & 3 \\
\gls{diffndp}   & \textcolor{darkgreen}{56{\tiny$\pm$3}} & \textcolor{darkgreen}{53{\tiny$\pm$1}} & \textcolor{darkgreen}{96{\tiny$\pm$1}} & 87{\tiny$\pm$3} & \textcolor{darkgreen}{82{\tiny$\pm$4}} & 4 \\
\gls{diffndp}-E & \textcolor{darkgreen}{60{\tiny$\pm$4}} & \textcolor{darkgreen}{53{\tiny$\pm$2}} & \textcolor{darkgreen}{97{\tiny$\pm$1}} & \textcolor{darkgreen}{91{\tiny$\pm$2}} & \textcolor{darkgreen}{85{\tiny$\pm$5}} & \textbf{5} \\
\cmidrule[1.5pt]{1-7}
\end{tabular}
}
\caption{\small Node classification accuracy (Roman-empire, Amazon-ratings) and AUROC (Minesweeper, Tolokers, Questions). The best performing models in each dataset are in green and get 1 score point, 0 otherwise.}
\label{tab:node-classification}
\end{table}
\egroup

==> tables/node_class_stats.tex <==
\begin{table}[htbp]
\small
\centering
\caption{\small Statistics of node classification datasets.}
\label{tab:node-class_stats}
\begin{tabular}{lccccc}
\cmidrule[1.5pt]{1-5}
\textbf{Dataset}     & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{\# Classes} &  $\boldsymbol{h(\gG)}$ \\
\midrule
% Texas                & 183               & 325               & 5                   & \checkmark        & 0.000  \\
% Cornell              & 183               & 298               & 5                   & \checkmark        & 0.150  \\
% Wisconsin            & 521               & 515               & 5                   & \checkmark        & 0.084  \\
% Chameleon            & 2,277             & 31,371            & 5                   & \xmark          & 0.042  \\
% Squirrel             & 5,201             & 198,353           & 5                   & \xmark          & 0.031  \\
Roman-Empire         & 22,662            & 32,927            & 18                             & 0.021  \\
Amazon-Ratings       & 24,492            & 93,050            & 5                            & 0.127  \\
Minesweeper          & 10,000            & 39,402            & 2                              & 0.009  \\
Tolokers             & 11,758            & 519,000           & 2                              & 0.180  \\
Questions            & 48,921            & 153,540           & 2                              & 0.079  \\
\cmidrule[1.5pt]{1-5}
\end{tabular}
\end{table}

==> tables/old_05.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}l|llllllll@{}}
\toprule
dataset       & asapool   & diffpool  & dmon      & edgepool  & graclus   & kmis      & mincut    & topk      \\ \midrule
Bench-hard    & 0.69±0.03 & 0.65±0.06 & 0.70±0.04 & 0.70±0.05 & 0.70±0.04 & 0.69±0.03 & 0.71±0.04 & 0.51±0.05 \\
COLLAB        & 0.70±0.01 & 0.67±0.02 & 0.67±0.02 & 0.71±0.00 & 0.70±0.01 & 0.68±0.02 & 0.67±0.02 & 0.70±0.02 \\
DD            & 0.73±0.06 & 0.78±0.04 & 0.78±0.04 & nan±nan   & 0.75±0.04 & 0.75±0.03 & 0.79±0.04 & 0.73±0.03 \\
ENZYMES       & 0.26±0.05 & 0.34±0.06 & 0.34±0.06 & nan±nan   & 0.30±0.08 & 0.32±0.05 & 0.29±0.05 & 0.26±0.05 \\
EXPWL1        & 0.99±0.01 & 0.71±0.02 & 0.71±0.02 & nan±nan   & 0.89±0.02 & 0.98±0.01 & 0.70±0.03 & 0.49±0.04 \\
MUTAG         & 0.78±0.10 & 0.81±0.11 & 0.84±0.12 & nan±nan   & 0.85±0.14 & 0.84±0.10 & 0.80±0.11 & 0.81±0.10 \\
Multipartite  & 0.09±0.01 & 0.10±0.02 & 0.44±0.03 & nan±nan   & 0.12±0.05 & 0.46±0.02 & 0.48±0.03 & 0.30±0.04 \\
Mutagenicity  & 0.77±0.03 & 0.78±0.02 & 0.78±0.02 & nan±nan   & 0.78±0.02 & 0.79±0.01 & 0.77±0.03 & 0.73±0.03 \\
NCI1          & 0.74±0.03 & 0.76±0.04 & 0.74±0.03 & nan±nan   & 0.75±0.03 & 0.75±0.02 & 0.74±0.03 & 0.72±0.02 \\
PROTEINS      & 0.73±0.07 & 0.75±0.05 & 0.76±0.04 & nan±nan   & 0.73±0.04 & 0.74±0.05 & 0.75±0.04 & 0.74±0.05 \\
REDDIT-B & 0.84±0.03 & 0.86±0.03 & 0.87±0.02 & nan±nan   & 0.86±0.02 & 0.87±0.03 & 0.84±0.03 & 0.87±0.03 \\ \bottomrule
\end{tabular}
\caption{Tabella pooling 0.5}
\end{table}

==> tables/others_0_1_stub_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}l|lllllllllll@{}}
\toprule
Pooling  & Bench-hard & COLLAB    & DD        & ENZYMES   & EXPWL1    & MUTAG     & Multipartite & Mutagenicity & NCI1      & PROTEINS  & REDDIT-BINARY \\ \midrule
asapool  & 0.51±0.05  & 0.70±0.01 & 0.71±0.03 & 0.23±0.04 & 0.58±0.12 & 0.69±0.13 & 0.39±0.03    & 0.74±0.03    & 0.70±0.02 & 0.72±0.04 & 0.80±0.03     \\
diffpool & 0.41±0.04  & 0.67±0.01 & 0.78±0.04 & 0.35±0.06 & 0.71±0.02 & 0.83±0.13 & 0.09±0.02    & 0.79±0.02    & 0.76±0.03 & 0.73±0.03 & 0.88±0.02     \\
dmon     & 0.70±0.05  & 0.67±0.01 & 0.78±0.04 & 0.35±0.06 & 0.71±0.02 & 0.81±0.14 & 0.39±0.03    & 0.78±0.02    & 0.76±0.02 & 0.75±0.05 & 0.88±0.03     \\
edgepool & 0.70±0.04  & 0.69±0.02 & nan±nan   & nan±nan   & nan±nan   & nan±nan   & nan±nan      & nan±nan      & nan±nan   & nan±nan   & nan±nan       \\
graclus  & 0.70±0.04  & 0.69±0.02 & 0.75±0.03 & 0.30±0.08 & 0.89±0.02 & 0.85±0.14 & 0.13±0.05    & 0.78±0.02    & 0.75±0.03 & 0.73±0.04 & 0.86±0.01     \\
kmis     & 0.69±0.03  & 0.68±0.02 & 0.75±0.03 & 0.32±0.05 & 0.98±0.01 & 0.84±0.10 & 0.46±0.02    & 0.78±0.02    & 0.75±0.02 & 0.74±0.05 & 0.87±0.02     \\
mincut   & 0.71±0.03  & 0.68±0.02 & 0.79±0.04 & 0.34±0.08 & 0.71±0.02 & 0.80±0.12 & 0.44±0.03    & 0.78±0.03    & 0.75±0.02 & 0.74±0.05 & 0.87±0.02     \\
topk     & 0.32±0.04  & 0.62±0.02 & 0.74±0.04 & 0.20±0.04 & 0.49±0.04 & 0.73±0.12 & 0.18±0.03    & 0.70±0.02    & 0.69±0.03 & 0.72±0.05 & 0.79±0.03     \\ \bottomrule
\end{tabular}
\caption{Tabella pooling 0.1}
\label{tab:res-1}
\end{table}

==> tables/pooling_drawbacks.tex <==

\bgroup
\def\arraystretch{1.0} %vertical padding 
\setlength\tabcolsep{1.1em} %horizontal padding
\begin{table}[htbp]
\small
\centering
\caption{\small Drawbacks of different types of pooling operators.}
\label{tab:drawbacks}
\begin{tabular}{@{}lll@{}}
\textbf{Soft-clustering} & \textbf{Score-based} & \textbf{One-every-$\boldsymbol{k}$} \\
\toprule
\xmark \; Not adaptive to graph size & \xmark \; Pooling not uniform & \xmark \; Limited flexibility \\
\xmark \; Dense and not interpretable pooled graphs & \xmark \; Not expressive & \xmark \; Task agnostic \\
\xmark \; High memory cost & \xmark \; Worse performance &  \\
\bottomrule
\end{tabular}
\end{table}
\egroup

==> tables_2025/graph_class_hp_exp.tex <==
\begin{table}[htbp]
\centering
\caption{Hyperparameters configurations of the AUX-Net for the graph classification task in the expressive case.}
\label{tab:graph-class_config_expr}
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-3}
\textbf{Dataset}     & MP units & $\beta$ \\
\midrule
GCB-H         & $[32] \times 8$ & 5.0 \\
COLLAB       & $[32] \times 8$ & 1.0 \\
DD          & $[8] \times 16$ & 5.0 \\
ENZYMES & $[16] \times 8$ & 3.0 \\
EXPWL1 & $[16] \times 8$ & 1.0 \\
MUTAG & $[16] \times 8$ & 3.0 \\
Multipartite & $[32] \times 8$ & 1.0 \\
Mutagenicity & $[32] \times 8$ & 5.0 \\
NCI1 & $[8] \times 16$ & 3.0 \\
PROTEINS & $[32, 32, 16, 16, 8, 8]$ & 5.0 \\
REDDIT-B & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 \\
\cmidrule[1.5pt]{1-3}
\end{tabular}
\end{table}


==> tables_2025/graph_class_hp_non_exp.tex <==
\begin{table}[htbp]
\centering
\caption{Hyperparameters configurations of the AUX-Net for the graph classification task in the non expressive case.}
\label{tab:graph-class_config}
\begin{tabular}{lcccc}
\cmidrule[1.5pt]{1-3}
\textbf{Dataset}     & MP units & $\beta$ \\
\midrule
GCB-H         & $[8] \times 16$ & 3.0 \\
COLLAB       & $[32] \times 8$ & 1.0 \\
DD          & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 1.0 \\
ENZYMES & $[8] \times 16$ & 3.0 \\
EXPWL1 & $[32,32,16,16,8,8]$ & 1.0 \\
MUTAG & $[8] \times 16$ & 1.0 \\
Multipartite & $[32] \times 8$ & 3.0 \\
Mutagenicity             & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
NCI1            & $[32, 32, 16, 16, 8, 8]$ & 1.0 \\
PROTEINS & $[32, 32, 32, 32, 16, 16, 16, 16, 8, 8, 8, 8]$ & 3.0 \\
REDDIT-B & $[32] \times 8$ & 1.0 \\
\cmidrule[1.5pt]{1-3}
\end{tabular}
\end{table}

